Efficient Neural Radiance Fields for Interactive Free-viewpoint Video

This paper aims to tackle the challenge of efficiently producing interactive free-viewpoint videos. Some recent works equip neural radiance fields with image encoders, enabling them to generalize across scenes. When processing dynamic scenes, they can simply treat each video frame as an individual scene and perform novel view synthesis to generate free-viewpoint videos. However, their rendering process is slow and cannot support interactive applications. A major factor is that they sample lots of points in empty space when inferring radiance fields. We propose a novel scene representation, called ENeRF, for the fast creation of interactive free-viewpoint videos. Specifically, given multi-view images at one frame, we first build the cascade cost volume to predict the coarse geometry of the scene. The coarse geometry allows us to sample few points near the scene surface, thereby significantly improving the rendering speed. This process is fully differentiable, enabling us to jointly learn the depth prediction and radiance field networks from RGB images. Experiments on multiple benchmarks show that our approach exhibits competitive performance while being at least 60 times faster than previous generalizable radiance field methods.

==> tables/ablation_training.tex <==
\begin{table}
  \centering
%   \tabcolsep=0.13cm
%   \setlength\tabcolsep{5.3pt}
\caption{\textbf{Image synthesis results on 4 frames of the ZJU-MoCap dataset in terms of PSNR metric.} ``Per-frame training'' means we simply fine-tune the pre-trained network on the test frame. ``Per-sequence training'' means we fine-tune the pre-trained network on the whole sequence. }

  \begin{tabular}{c|cccc|c}
    \toprule
    Test frame id & 1 & 2 & 3 & 4 & Mean \\
    % \midrule
    \hline
    Per-frame training  & 36.73 & 33.07 & 34.46 & 33.24 & 34.38 \\
    Per-sequence training  & 37.68 & 35.55 & 36.33 & 35.30 & 36.22  \\
    \bottomrule
  \end{tabular}
  
\label{tab:ablation_training}
\end{table}

==> tables/comp_dtu_syn.tex <==
\begin{table}
\tabcolsep=0.06cm
\begin{center}
\caption{\textbf{Comparisons with generalizable radiance field methods.} The rendering image resolutions of DTU and NeRF Synthetic are $512 \times 640$ and $800 \times 800 $, respectively. To report the rendering speed, we set the rendering resolution to $512 \times 512$. }
\label{tab:dtu_syn}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|ccc|c}

\Xhline{3\arrayrulewidth}
 & \multicolumn{3}{c|}{DTU } & \multicolumn{3}{c|}{NeRF Synthetic}  \\ 
\hline
%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FPS  $\uparrow$ \\
  & PSNR  & SSIM & LPIPS  & PSNR  & SSIM  & LPIPS  & FPS  \\
\hline
PixelNeRF & 19.31 & 0.789 & 0.382 & 7.39 & 0.658 & 0.411 & 0.019 \\
IBRNet  & 26.04 & 0.917 & 0.191 & 22.44 & 0.874 & 0.195 & 0.217 \\
MVSNeRF & 26.63 & 0.931 &  0.168 & 23.62 & 0.897 & 0.176 & 0.416 \\
Ours & \textbf{27.61} & \textbf{0.956} & \textbf{0.091} & \textbf{26.65} &  \textbf{0.947} & \textbf{0.072} & 25.29 \\
\hline
NeRF (10.2h) & 27.01 & 0.902 & 0.263 & 30.63 & 0.962 & 0.093 \\
\hline
IBRNet (1h) & 31.35 & 0.956 & 0.131 & 25.62 & 0.939 &  0.111 & 0.217  \\
MVSNeRF (15min) & 28.51 & 0.933 & 0.179 & 27.07 & 0.931 &  0.168 & 0.416\\
Ours (15min) & 30.12 & 0.963 & 0.079 & 27.20 & 0.951 &  0.066 &  25.29  \\
Ours (1h) & \textbf{31.41} & \textbf{0.967} & \textbf{0.069} & \textbf{27.57} & \textbf{0.954} & \textbf{0.063} &  25.29  \\
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{center}

% \vspace{-1em}

\end{table}

==> tables/comp_zjumocap.tex <==
% \begin{table*}
%   \centering
% %   \tabcolsep=0.15cm
% %   \setlength\tabcolsep{5.3pt}
% \scalebox{0.95}{
%   \begin{tabular}{llllllllll}
%     \toprule
%     \multirow{2}{*}{Methods} & 
%     \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Training \\ h /1200 frames\end{tabular}} &
%     \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Extra storage \\ GB /1200 frames\end{tabular}} &
%     \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}} FPS \\ 512x512\end{tabular}} &
%     \multicolumn{6}{c}{ZJU-MoCap~\cite{peng2021neural}} \\
%     \cmidrule(lr){5-10}
%     & & & & F.0001 & F.0400 & F.1175 & F.1200 & Mean & All \\
%     \midrule
%     NeRF~\cite{mildenhall2020nerf} & 2.5 * 1200 $^\dag$ & 0  & 0.10 & 38.01 & 35.07 & 35.92 & 33.85 & 35.71 & -- \\
%     PlenOctree~\cite{yu2021plenoctrees} & 4 * 1200 $^\dag$ & 1.45 * 1200 $^\dag$ & 150 & 37.21 & 34.62 & 34.11 &  33.47 & 34.85& --\\
%     NeuralBody~\cite{peng2021neural} & 12 & 0 & & 35.91 & 32.34 & 34.58 & 32.75 & 33.90 & 34.38\\
%     Ours & 0 & 0 & 19.04 & 34.83 &  32.89 & 32.66 & 31.91 & 33.07 & 33.16\\
%     Ours-ft & 8 & 0 & 19.04 & 37.68 & 35.55 & 36.33 & 35.30 & 36.22 & 36.21\\
    
%     \bottomrule
%   \end{tabular}}
%   \caption{Quantitative comparison of per-scene fine-tuning image synthesis results on datasets of DTU~\cite{jensen2014large}, Real Forward-Facing~\cite{mildenhall2020nerf} and NeRF Synthetic~\cite{mildenhall2020nerf}.}
% \label{tab:comp_zjumocap}
% \end{table*}


% \begin{table}
%   \centering
%   \tabcolsep=0.13cm
% %   \setlength\tabcolsep{5.3pt}
% \scalebox{0.95}{
%   \begin{tabular}{lcccc}
%     \toprule
%     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods \end{tabular}}  & 
%     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Storage\end{tabular}}  &
%     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training \\ time \end{tabular}}  &
%     \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rendering \\ FPS $\uparrow$ \end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PSNR$\uparrow$ \end{tabular}}  \\
%     & & & & \\
%     \midrule
%     NeRF~\cite{mildenhall2020nerf} & 5.39$^\dag$ & 3000$^\dag$  & 0.10 & 35.71 \\
%     PlenOctree~\cite{yu2021plenoctrees} & 1740$^\dag$ & 4800$^\dag$ & \textbf{150} & 34.85 \\
%     NeuralBody~\cite{peng2021neural} & 0.018 & 12 & 5.49 & 33.90 \\
%     Ours & 9.67 & 0 & 19.04 & 33.07 \\
%     Ours$_{ft}$ & 9.67 & 8 & 19.04 & \textbf{36.22}\\
    
%     \bottomrule
%   \end{tabular}}
%   \caption{Quantitative comparison of image synthesis results on the ZJU-MoCap~\cite{peng2021neural} dataset. Results$^\dag$ means that we only test for 4 frames because of its expensive cost. Then we calculate the average cost and expand it to 1200 frames. The units of ``Storage'' and ``Training time'' are GB and hours, respectively. ``Ours'' represents the proposed method which are pretrained on the DTU~\cite{jensen2014large} dataset. Ours$_{ft}$ means we finetune the pretrained model on this dynamic scene of the ZJU-MoCap dataset.}
% \label{tab:comp_zjumocap}
% \end{table}


\begin{table}
  \centering
  \vspace{-3mm}
%   \tabcolsep=0.13cm
%   \setlength\tabcolsep{5.3pt}
  \caption{\textbf{Quantitative comparison on the ZJU-MoCap dataset.} The units of ``Storage'' and ``Preprocess time'' are in GB and hours, respectively. 
  ``Ours'' and ``Ours$_{ft}$ '' respectively represent the models trained on the DTU dataset and fine-tuned on this dynamic scene.
%   ``Ours'' represents the proposed method trained on the DTU~\cite{jensen2014large} dataset. Ours$_{ft}$ means we finetune the pre-trained model on this dynamic scene. 
%   The rendered image resolution is 512 $\times$ 512. 
  To obtain the results of~\cite{yu2021plenoctrees}, we test it only on 4 frames and multiply the average cost by 1200 frames, because of its expensive cost.}
% \scalebox{0.95}{
  \begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Methods \end{tabular}}  & 
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Storage\end{tabular}}  &
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Preprocess \\ time \end{tabular}}  &
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rendering \\ FPS $\uparrow$ \end{tabular}}  & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}PSNR$\uparrow$ \end{tabular}}  \\
    & & & & \\
    \midrule
    % NeRF~\cite{mildenhall2020nerf} & 5.39$^\dag$ & 3000$^\dag$  & 0.10 & 35.71 \\
    PlenOctree & 1740 & 1800 & \textbf{150} & 34.85 \\
    NeuralBody & 0.018 & -- & 5.49 & 33.90 \\
    Ours & 0.47 & -- & 19.04 & 33.07 \\
    Ours$_{ft}$ & 0.47 & -- & 19.04 & \textbf{36.22}\\
    
    \bottomrule
  \end{tabular}
%   }
%   \caption{Quantitative comparison on the ZJU-MoCap~\cite{peng2021neural} dataset. The units of ``Storage'' and ``Preprocess time'' are in GB and hours, respectively. ``Ours'' represents the proposed method trained on the DTU~\cite{jensen2014large} dataset. Ours$_{ft}$ means we finetune the pre-trained model on this dynamic scene. The 
%  rendered image resolution is $512 \times 512$. To obtain the results of~\cite{yu2021plenoctrees}, we test it only on 4 frames and multiply the average cost by 1200 frames, because of its expensive cost.}
\vspace{-1mm}
\label{tab:comp_zjumocap}
\end{table}


==> tables/nomask_setting.tex <==
\begin{table}
\tabcolsep=0.2cm
\begin{center}
\caption{\textbf{Quantitative results on the ZJU-MoCap Part II dataset.} }
\label{table:nomask}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc|c}
\Xhline{3\arrayrulewidth}
%  & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & FPS  $\uparrow$ \\
  & PSNR $\uparrow$ & SSIM  $\uparrow$ & LPIPS  $\downarrow$   & FPS $\uparrow$ \\
\hline
STNeRF (20h) & 25.30 & 0.935 & 0.407  &  \\
IBRNet (0h) & 21.91 & 0.900  & 0.461  & 0.217 \\
IBRNet (2h) & 23.39 & 0.920  & 0.437 & 0.217 \\
\hline
Ours (0) & 22.59 & 0.922 & 0.306 & 28.99 \\
Ours (15min) & 23.69 & 0.942 & 0.237 & 28.99 \\
Ours (2h) & \textbf{23.95} & \textbf{0.943} & \textbf{0.224}  & 28.99\\
\hline
w/o Composition (0) & 21.90 & 0.896 & 0.370 & 30.57 \\
w/o Composition (2h) & 23.70 & 0.928 & 0.310 & 30.57 \\
% w/o bg images (0) & 22.11 & 0.901 & 0.364 & 28.99 \\
% w/o bg images (2h) & 23.78 & 0.937 & 0.224 & 28.99 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{center}

% \vspace{-1em}

\end{table}

